Active and sparse methods in smoothed model checking

Smoothed model checking based on Gaussian process classification provides a powerful approach for statistical model checking of parametric continuous time Markov chain models. The method constructs a model for the functional dependence of satisfaction probability on the Markov chain parameters. This is done via Gaussian process inference methods from a limited number of observations for different parameter combinations. In this work we consider extensions to smoothed model checking based on sparse variational methods and active learning. Both are used successfully to improve the scalability of smoothed model checking. In particular, we see that active learning-based ideas for iteratively querying the simulation model for observations can be used to steer the model-checking to more informative areas of the parameter space and thus improve sample efficiency. Online extensions of sparse variational Gaussian process inference algorithms are demonstrated to provide a scalable method for implementing active learning approaches for smoothed model checking.

==> takeout.tex <==
%\section{Random linear embeddings}
%The shape and properties of the parameter spaces of pCMTC models are generally
%logical specification.
%For example, not all directions in the parameter space are made equal and
%the satisfaction probability can be non-stiff with respect to parameter changes
%in one direction while being stiff with respect changes in another.
%%That is, models can exhibit sloppyness as introduced in the context of systems
%%biology models~\cite{GutenkunstWCBMS07}. 
%%
%Understanding this has implications in various applications of model checking. 
%For example, in the context of parameter synthesis from logical specification,
%knowing the non-stiff parts of the parameter space helps us to concentrate the
%optimisation efforts to the parts of the parameter space where the synthesised
%parameters can be hoped to be robust with respect to parameter fluctuations.
%%Here we are going to start by exploring a related aspect and attempt to   
%%Similarly, by adaptively identifying the non-stiff parts of the parameter space 
%%allows to us to 
%
%Our approach is going to be based on random linear embeddings of the parameter
%space.
%We start by introducing a simple example from~\cite{BortolussiMS16}.
%\begin{example}
%As an example we start by considering a simple SIR model  
%\begin{align*}
%    S + I & \xrightarrow{k_I} I + I \\
%    I & \xrightarrow{k_R} R
%\end{align*}
%where $S$ gives the number of susceptible, $I$ the infected and $R$ the
%recovered individuals in the system. 
%For initial conditions we set $(95, 5, 0)$. 
%That is at time zero there are $95$ susceptible, $5$ infected and $0$ recovered.
%The parameters $k_I$ and $k_R$ give the infection and recovery rates
%respectively.
%\end{example}
%
%The property we are going to consider is the following: 
%Constraining the parameters to the ranges $k_I \in [0.005, 0.3]$ and $k_R \in
%[0.005, 0.3]$ gives satisfaction probabilities depicted in the
%Figure~\ref{fig:baseline-surface}.
%The each estimate on the $20$-by-$20$ grid is calculated based on $1000$
%stochastic simulation sample runs of the model.
%For comparison Figure~\ref{fig:smoothed-surface} gives the results of the
%smoothed model checking where $10$ sample trajectories are drawn for each
%parameter on the $20$-by-$20$ grid.
%Note that even in this simple case a significant amount of sampling is done in
%parts of the parameter space where the satisfaction probability remains close to
%$0$.
%
%The idea for overcoming this is to consider random linear embeddings based
%sampling of the parameters space. 
%Methods based on random linear embedding have been proposed to deal with high
%dimensional Bayesian optimisation problems where the effective dimensionality 
%is low~\cite{WangHZMF16}.
%That is there is a low dimensional subspace of the parameter space which governs
%the behaviour of the function that is optimised.
%Here, the situation is different as we can see from the baseline SSA based
%surface in Figure~\ref{fig:baseline-surface} that the model checking problem
%remains two dimensional.
%
%\todo{Idea I'm trying to make work is the following: 
%\begin{itemize}
%    \item sample a line going through the parameter space
%    \item gather single-trajectory model checking samples for parameters on the
%        line
%    \item how informative sampling from this line is can be decided based of
%        Shannon entropy calculated for the empirical distribution of
%        the model-checking outcomes. That is, we have a proportion of true and
%        false values observed on the line. 
%        Empirical probability of seeing true on the line close to $1/2$ would mean
%        we are on a line where we might want to sample more on the same line.
%        While empirical probability of seeing true close to 0 or 1 means we
%        probably don't need to sample more on that line.  
%    \item still unclear how exactly to sample a new line based on the entropy
%        calculations.
%\end{itemize}
%}
%%\begin{itemize}
%%    \item initialise a random line through the parameter space. 
%%    \item use samples on this line to calculate the posterior of the smoothed
%%        model checking problem in Section~\ref{sec:model checking}.
%%\end{itemize}
%
%\begin{figure}
%    \centering
%    \begin{subfigure}[t]{0.49\textwidth}
%        \includegraphics[width=\textwidth]{figures/baseline_grid.pdf}
%        \caption{Baseline satisfaction probability surface}
%        \label{fig:baseline-surface}
%    \end{subfigure}
%    \begin{subfigure}[t]{0.49\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{figures/smoothed_grid.pdf}
%        \caption{Smoothed model checking satisfaction probability surface}
%        \label{fig:smoothed-surface}
%    \end{subfigure}
%
%    \begin{subfigure}[t]{0.49\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{figures/smoothed_random.pdf}
%        \caption{Smoothed model checking sampling from random lines}
%        \label{fig:smoothed-surface}
%        \todo{The last one is just sampling data points from random lines. No search strategy yet.}
%    \end{subfigure}
%
%    \caption{Satisfaction probability surfaces}
%\end{figure}


%\section{Acquisition functions}
%An important concept in bayesian optimisation is that of an acquisition
%function.
%An acquisition function guides the exploration of the parameter space.
%The construction of the functions has to deal with the trade-off between
%exploration and exploitation by weighing whether unexplored regions or regions
%around known optima should be prioritised for new samples.
%\todo{Observations are noisy. The entropy based approach gives us a way to
%decide where the small set of trajectories are expected to have the most effect?} 
%

